Energy-Based Imitation Learning

We tackle a common scenario in imitation learning (IL), where agents try to recover the optimal policy from expert demonstrations without further access to the expert or environment reward signals. Except the simple Behavior Cloning (BC) that adopts supervised learning followed by the problem of compounding error, previous solutions like inverse reinforcement learning (IRL) and recent generative adversarial methods involve a bi-level or alternating optimization for updating the reward function and the policy, suffering from high computational cost and training instability. Inspired by recent progress in energy-based model (EBM), in this paper, we propose a simplified IL framework named Energy-Based Imitation Learning (EBIL). Instead of updating the reward and policy iteratively, EBIL breaks out of the traditional IRL paradigm by a simple and flexible two-stage solution: first estimating the expert energy as the surrogate reward function through score matching, then utilizing such a reward for learning the policy by reinforcement learning algorithms. EBIL combines the idea of both EBM and occupancy measure matching, and via theoretic analysis we reveal that EBIL and Max-Entropy IRL (MaxEnt IRL) approaches are two sides of the same coin, and thus EBIL could be an alternative of adversarial IRL methods. Extensive experiments on qualitative and quantitative evaluations indicate that EBIL is able to recover meaningful and interpretative reward signals while achieving effective and comparable performance against existing algorithms on IL benchmarks.

==> papers/5-related.tex <==
\section{Related Work}
\subsection{Imitation Learning}
As extensions for the traditional solution as inverse reinforcement learning~\cite{ng2000algorithms,abbeel2004apprenticeship,fu2017learning}, generative adversarial algorithms raised up these days. Begin with GAIL~\cite{ho2016generative}, which model the imitation learning as an occupancy measure matching problem, and takes a GAN-form objective to optimize both the reward and the policy. AIRL~\cite{fu2017learning} simplifies the idea of \cite{finn2016connection} and use a disentangled discriminator to recover the reward function in an energy-form. However, as we show in experiments, they do not actually recover the energy. Conclude from previous works, \cite{ke2019imitation} and \cite{ghasemipour2019divergence} concurrently propose to unify the adversarial learning algorithms with f-divergence, like \cite{nowozin2016f}, they claim that any f-divergence can be used to construct a generative adversarial imitation learning algorithm. Specifically, \cite{ghasemipour2019divergence} propose FAIRL, which adopts the forward KL as the distance metric.

Instead of seeking to alternatively update the policy and the reward function as in IRL and GAIL, many recent works of IL aim to learn a fixed reward function directly from expert demonstrations and then apply a normal reinforcement learning procedure with that reward function. This idea can be found inherently in previous GMMIL work~\cite{kim2018imitation} that utilizes the maximum mean discrepancy as the distance metric to guide training. Recently, \cite{wang2019red} propose Random Expert Distillation (RED), which employs the idea of Random Network Distillation\cite{burda2018rnd} to compute the reward function by the loss of fitting a random neural network or an auto-encoder. \cite{reddy2019softqil} applies constant rewards by setting positive rewards for the expert state-actions and zero rewards for other ones, which is optimized with the off-policy SQL algorithm~\cite{haarnoja2018soft}. In addition, Disagreement-Regularized Imitation Learning (DRIL) \cite{brantley2020disagreementregularized} constructs the reward function using the disagreement in their predictions of an ensemble of policies trained on the demonstration data, which is optimized together with a supervised behavioral cloning cost. 
These works resembles the idea of EBIL, where the reward function can be seen as approximated energy functions. For example, in \cite{wang2019red} propose an alternative for estimating the reward using an auto-encoder, which is exactly the way of energy modeling in EBGAN~\cite{zhao2016energy}; In addition, \cite{wang2019red} and \cite{brantley2020disagreementregularized} also utilize the prediction errors, which are high on demonstration data but low on data that is out of the demonstration. \cite{reddy2019softqil} is more straightforward that simply set the energy of the expert as 0 and the agent's as 1. However, theses approximated energies are not derived from statistical modeling and lack the theoretical 
correctness. Beside these methods, \cite{kostrikov2019imitation} proposed valueDICE, which solves imitation learning via off-policy distribution ratio estimation without a separate RL optimization. valueDICE overcomes the on-policy limitation of previous alternative optimization methods as GAIL and IRL, which is required access to on-policy samples. However, with our two-stage training style and a independent policy learning stage, we are free to combine any on-policy or off-policy RL learning algorithms. It is worth noting that combining the idea of EBGAN~\cite{zhao2016energy} and GAIL~\cite{ho2016generative} we can also design an adversarial style energy-based algorithm for imitation learning, however it is less interesting and also does not have statistical support about the learned energy.

\subsection{Energy-Based Modeling}
Our EBIL relies highly on EBMs, which have played an important role in a wide range of tasks including image modeling, trajectory modeling and continual online learning \cite{Du2019generalization}. 
%works based on EBMs such as \cite{grathwohl2020classfierisEBM} can make breakthroughs.
Thanks to the appealing features, EBMs have been introduced into many RL literature, for instance, parameterized as value function~\cite{sallans2004valueEBM}, employed in the actor-critic framework~\cite{heess2012acEBMs}, applied to MaxEnt RL~\cite{haarnoja2017reinforcement} and model-based RL regularization~\cite{boney2019regularizing}. 
%\cite{finn2016connection} also reveals the connection between IRL and EBMs.
However, EBMs are always difficult to train due to the partition function \cite{finn2016connection}. Nevertheless, recent works have tackled the problem of training large-scale EBMs on high-dimensional data, such as DEEN~\cite{saremi2018deep} which is applied in our implementation. Except for DEEN, there still leaves plenty of choices for efficiently training EBMs \cite{gutmann2012noise,Du2019generalization,nijkamp2019learn}. 


==> papers/6-exp.tex <==
\section{Experiments}

In this section we seek to empirically evaluate EBIL to figure out the effectiveness of our solution compared to previous works, especially the alternative optimization methods. We first conduct qualitative and quantitative experiments on a simple one-dimensional environment, where we illustrate the recovered reward in the whole state-action space and show the training stability of EBIL. Then, we test EBIL against baselines on benchmark environments using sub-optimal experts and release competitive performance.

\subsection{Synthetic Task}
\label{sec:one-domain}

\begin{figure}
%\vspace{-7pt}
\includegraphics[width=0.8\linewidth]{figs/KL-crop.pdf}
\vspace{-2pt}
\caption{The KL divergence between the agent trajectories and the expert during the learning procedure, which indicates that EBIL is much more stable than the other methods. The blue dash line represents the converged result of EBIL.}
\vspace{-14pt}
\label{fig:kl-div}
\end{figure}

In the synthetic task, we want to evaluate the qualitative performance of different IL methods by displaying the heat map of the learned reward signals and sampled trajectories. 
We want EBIL to be capable of guiding the agent to recover the expert policy and correspondingly generate the high-quality trajectories. Therefore, we evaluate EBIL on a synthetic environment where the agent tries to move in a one-dimensional space. 
Specifically, the state space is $[ -0.5, 10.5 ]$ and the action space is $[-1, 1]$. The environment initializes the state at $0$, and we set the expert policy as static rule policies $\pi_E = \gN(0.25, 0.06)$ when the state $s\in [ -0.5, 5 )$, and $\pi_E = \gN(0.75, 0.06)$ when $s\in [ 5, 10.5 ]$. The sampled expert demonstration contains $40$ trajectories with up to $30$ timesteps in each one. 
For all methods, we choose SAC \cite{haarnoja2018soft} as the learning algorithm and we continue training each algorithm until convergence.

In this illustrative experiment, we compare EBIL aginst GAIL~\cite{ho2016generative}, AIRL~\cite{fu2017learning} and RED~\cite{wang2019red}, where GAIL and AIRL are two representative works of adversarial imitation learning which take an alternative updating on the reward and the policy. RED resembles EBIL which also take a two-stage training by first estimate the reward through the prediction error of a trained network with a randomized one. We plot the KL divergence between the agent's and the expert's trajectories during the training procedure in \fig{fig:kl-div} and visualize the final estimated rewards with corresponding induced trajectories in \fig{fig:heat_maps}.

As illustrated in \fig{fig:ebil_heat} and \fig{fig:kl-div}, the pre-estimated reward of EBIL successfully captures the density of the expert trajectories, and leaded by the interpretative reward the induced policy is able to quickly converge to the expert policy. By contrast, GAIL requires a noisy adversarial process to correct the policy. As a result, although GAIL achieves compatible final performance against EBIL~(\fig{fig:gail_heat}), it suffers a slow, unstable training as shown in \fig{fig:kl-div} and assigns meaningless reward in the state-action space, as revealed in \fig{fig:gail_heat}.
In addition, we are surprised to find that AIRL recovers an `inverse'-type reward signals but can also learns well, as suggested in \fig{fig:airl_heat}. We analyse such a problem in \se{ap:airl}, where we conclude that AIRL actually does not recover the energy of experts but the energy with an entropy term. Removing such an entropy term makes the result more reasonable. Finally, we notice that constructing the reward as the prediction errors does not help to recover a meaningful signal, as shown in \fig{fig:red_heat}, where RED suffers from the diverged reward and fails to imitate the expert accurately.

On the contrary, EBIL benefits from meaningful rewards which is tend to learn a deterministic policy which shows the most likelihood. Thus, the recovered policy has less variance but the mean is very close to the expert, which is a good property. In fact, a optimal policy is usually a deterministic policy due to bellman equation and a stochastic policy is always used to increase the exploration ability in a learning procedure. the exploration ability is much necesarry for methods as EBIL and RED. Although it is convincing to take the recovered energy as a meaningful reward signal for imitation learning, we must point out that as illustrated in \fig{fig:ebil_heat}, the recovered reward maybe be sparse in the space where the expert scarcely comes by. Thus, to gain better performance, the agents will be required to equip with an efficient RL algorithm with good exploration ability.

\begin{figure*}[!t]
\centering
\subfigure[Expert Trajectories]{
\begin{minipage}[b]{0.28\linewidth}
\label{fig:expert_heat}

\includegraphics[width=1\linewidth]{figs/heat-crop/expert-crop.pdf}
\vspace{-0.8pt}
\end{minipage}
}
\hspace{-10pt}
\subfigure[EBIL]{
\begin{minipage}[b]{0.155\linewidth}
\label{fig:ebil_heat}
\includegraphics[width=1\linewidth]{figs/heat-crop/ebil_reward_heat_40-crop.pdf}
\includegraphics[width=1\linewidth]{figs/heat-crop/[1724_34]ebil_agent_heat_40_667-crop.pdf}
\end{minipage}
}
\subfigure[GAIL]{
\begin{minipage}[b]{0.155\linewidth}
\label{fig:gail_heat}
\includegraphics[width=1\linewidth]{figs/heat-crop/gail_heat_40_19890-crop.pdf}
\includegraphics[width=1\linewidth]{figs/heat-crop/[3124_52]gail_agent_heat_40_15000-crop.pdf}
\end{minipage}
}
\subfigure[AIRL]{
\begin{minipage}[b]{0.155\linewidth}
\label{fig:airl_heat}
\includegraphics[width=1\linewidth]{figs/heat-crop/airl_heat_40_16000_1-crop.pdf}
\includegraphics[width=1\linewidth]{figs/heat-crop/[4196_12]airl_agent_heat_40_16000-crop.pdf}
\end{minipage}
}
\subfigure[RED]{
\begin{minipage}[b]{0.155\linewidth}
\label{fig:red_heat}
\includegraphics[width=1\linewidth]{figs/heat-crop/rnd_heat_40_499-crop.pdf}
\includegraphics[width=1\linewidth]{figs/heat-crop/[23968_43]rnd_agent_heat_40_19999-crop.pdf}
\end{minipage}
}
\vspace{-3pt}
\caption{Heat maps of the expert trajectories (leftmost), the (final) \textit{estimated rewards} recovered by different methods (top) and the corresponding \textit{induced policy} (bottom). The horizontal and the vertical axis denote the \textit{state space} and the \textit{action space} respectively. The red dotted line represents the position where the agent should change its policy. 
It is worth noting that EBIL and RED both learn fixed reward functions, while GAIL and AIRL iteratively update the reward signals. We do not compare BC since it learns the policy via supervised learning without recovering any reward signals.}
\vspace{-2pt}
\label{fig:heat_maps}
\end{figure*}

%will learn little if they are in those spaces since the learned energy will provide less information. Thus an efficient RL algorithm with good exploration ability is required. This scenario may be common for tasks with high-dimensional state-action space and a small amount of data.


\subsection{Imitation on Continous Control Benchmarks}

\paragraph{Sub-optimal Experts}

We also conduct evaluation experiments on the standard continuous control benchmarking MuJoCo environments. For each task, we train experts with OpenAI baselines version~\cite{dhariwal2016openai} of Proximal Policy Optimization (PPO)~\cite{schulman2017proximal} and get sub-optimal demonstrations. We employ Trust Region Policy Optimization (TRPO)~\cite{schulman2015trust} as the learning algorithm in the implementation for all evaluated methods, and we do not apply BC initialization for all tasks. We consider 4 demonstrated trajectories by the sub-optimal expert, as \cite{ho2016generative,wang2019red} do. We compare EBIL with several baseline methods and report the \textit{converged} result in \tb{tab:mujoco}, which are evaluated throughout 50 test episodes. % For GAIL and AIRL, we use a 3 layer MLP model for the discriminator as the energy model used in EBIL.
%The training curves are shown in \ap{ap:exp}, showing the training stability of the algorithm.

As shown in \tb{tab:mujoco}, with sub-optimal demonstrations, EBIL can achieve the best or comparable performance among all environments, indicating that the recovered energy is able to become a good reward signal for imitating the experts. However, learning from such a sub-optimal expert seems challenging for GAIL and AIRL, which are less robust to reach a better performance. We notice that on some environment as InvertedDoublePendulum, GAIL and AIRL can work during the training, but does not converge until the end. We think the problem is due to the training instability of GAN, which always need an early stop to get a better performance. On the contrary, EBIL provide steady reward signals  instead of a alternative trained one that stabilizes the training. The performance of RED and GMMIL also indicates that the recovered reward by random distillation or the maximum mean discrepancy do not provide a stable guidance in such an sub-optimal setting. However, benefit from such a steady reward function, RED and GMMIL can perform better than GAIL and AIRL on some tasks.

\begin{table*}[t]
\vskip 0.15in
\caption{Comparison for different methods of the episodic true rewards with sub-optimal demonstrations on 5 continuous control benchmarks. The means and the standard deviations are evaluated over different random seeds.}
\begin{center}
\begin{tabular}{cccccc}
\toprule
Method & Humanoid & Hopper & Walker2d & Swimmer & InvertedDoublePendulum\\
\midrule
Random & 100.38 $\pm$ 28.25 & 14.21 $\pm$ 11.20 & 0.18 $\pm$ 4.35 & 0.89 $\pm$ 10.96 & 49.57 $\pm$ 16.88 \\
\hline
BC & 178.74 $\pm$ 55.88 & 28.04 $\pm$ 2.73 & 312.04 $\pm$ 83.83 & 5.93 $\pm$ 16.77 & 138.81 $\pm$ 39.99\\
GAIL & 299.52 $\pm$ 81.52  & \textbf{1673.32 $\pm$ 57.13}  & 329.01 $\pm$ 211.84  & 23.79 $\pm$ 21.84  & 327.42 $\pm$ 94.92 \\
AIRL & 286.63 $\pm$ 6.05 & 126.92 $\pm$ 62.39  & 215.79 $\pm$ 23.04  & -13.44 $\pm$ 2.69 & 76.78 $\pm$ 19.63 \\
GMMIL & 416.83 $\pm$ 59.46 & 1000.87 $\pm$ 0.87 & 1585.91 $\pm$ 575.72 & -0.73 $\pm$ 3.28 & 4244.63 $\pm$ 3228.14\\
RED & 140.23 $\pm$ 19.10 & 641.08 $\pm$ 2.24 & 641.13 $\pm$ 2.75 & -3.55 $\pm$ 5.05 & 6400.19 $\pm$ 4302.03 \\
\textbf{EBIL} & \textbf{472.22 $\pm$ 107.72} & 1040.99 $\pm$ 0.53 & \textbf{2334.55 $\pm$ 633.91} & \textbf{58.09 $\pm$ 2.03} & \textbf{8988.37$\pm$ 1812.76}\\
\hline
Expert (PPO) & 1515.36 $\pm$ 683.59 & 1407.36 $\pm$ 176.91 & 2637.27 $\pm$ 1757.72 &  122.09  $\pm$ 2.60 &  6129.10 $\pm$ 3491.47 \\
\bottomrule
\end{tabular}
\label{tab:mujoco}
\end{center}
%\vskip -0.1in
\end{table*}

\paragraph{Optimal Demonstrations}

We also want to know how EBIL performs on optimal demonstrations compared with previous methods, especially adversarial inverse reinforcement learning methods such as GAIL, AIRL and FAIRL. 
Therefore we evaluate EBIL on optimal demonstrations from \cite{ghasemipour2019divergence}, where the expert is trained by SAC. As before, the demonstration for each task contains 4 trajectories and each trajectory is subsampled by a factor of 20. Similar to \cite{ghasemipour2019divergence}, we finetune each model and checkpoint the model at its \textit{best} validation loss and report the best resulting checkpoints on 50 test episodes. As shown in \tb{tab:mujoco-optimal}, we find that those adversarial algorithms can always achieves better performances on high-dimensional tasks as Hopper and Walker2d, where EBIL remains a gap between these methods. We think this problem is due to the accuracy of the energy model trained by DEEN, which only takes a simple MLP without further regularization operations. We must admit that benefiting from the various improvements of GAN such as gradient penelty~\cite{gulrajani2017improved} that makes the training more stable, adversarial algorithms has advantages than the traditional statistical modeling of EBMs, especially in high-dimensional space, since they can continue to improve the learning of data distribution in the iterative training procedure, while score matching methods as DEEN only model the provided dataset. 
However, on an easier environment LunarLander where the EBM can provide much meaningful and dense rewards, EBIL outperform the others while all the three adversarial algorithms have large variances. 

\begin{table}[htbp]
\vskip 0.15in
\caption{Comparison for different methods of the episodic true rewards with optimal demonstrations on 3 continuous control benchmarks. The means and the standard deviations are evaluated over different random seeds. We notice that EBIL can work better than adversarial inverse reinforcement learning algorithms on low-dimensional environments as LunarLander but remains performance gaps on harder tasks as Hopper and Walker2d.}
\begin{center}
\begin{tabular}{cccccc}
\toprule
Method & LunarLander & Hopper & Walker2d \\
\hline
Random & -232.81 $\pm$ 139.72 & 14.21 $\pm$ 11.20 & 0.18 $\pm$ 4.35 \\
\midrule
GAIL & -85.85 $\pm$ 59.22  & 3117.50 $\pm$ 2.96  & 4092.86 $\pm$ 7.46 \\
AIRL & -66.07 $\pm$ 104.14 & 3398.72 $\pm$ 8.39  & 3987.23  $\pm$ 334.04 \\
FAIRL & -116.90 $\pm$ 15.79 & 3353.78 $\pm$ 9.12  & 4225.66  $\pm$ 65.11 \\
\textbf{EBIL} & 237.95 $\pm$ 44.96 & 2401.93 $\pm$ 6.85 & 3026.60 $\pm$ 57.14 \\ %4563.03 $\pm$ 9.26\\
\hline
Expert & 254.90 $\pm$ 24.11 & 3285.92 $\pm$ 2.14 & 4807.22 $\pm$ 166.35\\
\bottomrule
\end{tabular}
\label{tab:mujoco-optimal}
\end{center}
%\vskip -0.1in
\vspace{-3pt}
\end{table}


\subsection{State Marginal Matching}

In this section we show that EBIL can also be helpful into matching the state marginal distributions for a given dataset. Motivated by \cite{ghasemipour2019divergence}, we try to make the agent learn the desired policy without expert demonstrations. Specifically, 
unlike the traditional IL setting, the target state marginal distribution does not even have to be a realizable state-marginal distribution collected by expensive expert demonstrations, but easy-to-get heuristically-designed interpretable distributions. Therefore, we test our methods in a 2D point mass task similar in ~\cite{ghasemipour2019divergence}, where agent can moves around the ground. We first generate 4000 heuristical samples as shown in \fig{fig:expert-smm}, learn the energy from them and then train the policy guided by the energy.

As expected, \fig{fig:energy-smm} illustrates that DEEN successfully recover the meaningful reward function, which describe the density of the target state marginal distribution. We then construct the reward function as $r(s) = h(-E(s))$ where $h$ is a monotonic linear function, with which the agent finally is able to induce similar trajectories to the expert. It is worth noted that we shape the recovered reward with an encourage on the exploration on the x-axis, since we find the with the state-only reward, the agent is tend to learn to go forth and back at the very beginning to the start point. Such a task remind us another possibility on finishing reinforcement learning tasks, where people do not have to carefully design the reward function but the samples on the desired trajectories. And by learning from the recovered energy of the provided samples with simple intuitive shaping that prevent the agent from cycling around, the agent can at last learn to complete the task.

\begin{figure}[htbp]
\centering
\includegraphics[width=0.49\columnwidth]{./figs/ablation-energy-hopper}
\includegraphics[width=0.49\columnwidth]{./figs/ablation-energy-walker}
\vspace{-7pt}
\caption{Ablation study on the average episode rewards evaluated on Hopper and Walker2dthat are learned with energy models from different training epochs using sub-optimal demonstrations , where the solid line and the shade represent the mean and the standard deviation on different runs separately.}
\vspace{-2pt}
\label{fig:ablation-energy}
\end{figure}

\subsection{Energy Evaluation}
\label{curves-energy}

EBIL relies highly on the training of EBMs which provide the reward to imitate the expert's policy. Therefore we have to evaluate the quality of a learned EBM before training the agent. However, the loss function of DEEN is not an intuitive indicator for evaluating the learned energy network, therefore, we propose to evaluate the averaged energy value for expert trajectories and the random trajectories on different tasks. As shown in \fig{fig:curves-energy}, DEEN finally converges in all experiments by successfully differentiating the expert dat from the random one. However, such a metric is a basic requirement and is always not that helpful on improving the performance of imitation learning, since the main difficulty comes from providing accurate reward signals for the trajectories that close to the experts. 

It is worth noting that in our experiments, we also find that a well-trained energy network may be hard for agents to learn the expert policies on some environments. 
We regard it as the ``sparse reward signals'' problem, as discussed in \se{sec:one-domain}. By contrast, sometimes a ``half-trained'' model may provide smoother rewards, and can help the agent to learn more efficiently. Actually, similar phenomenon also occurs when training the discriminator in GAN. We further analyze the training performance with energy models of different epochs in ablation study \se{sec:abl-study}.

\subsection{Ablation Study}
\label{sec:abl-study}

As mentioned before, to further understand the effect of the energy model from different training epochs, we conduct ablation study on energy models trained from different epochs. The results are illustrated in \fig{fig:ablation-energy}, which verify our intuition that a ``half-trained'' model can provide smoother rewards that solve the "sparse reward`` problem, which is better for imitating the expert policy.


\begin{figure*}[htbp]
\centering
\subfigure[Target State Marginal Distribution]{
\begin{minipage}[b]{0.3\linewidth}
\label{fig:expert-smm}
\includegraphics[width=1\linewidth]{./figs/smm/expert_triangle}
\end{minipage}
}
\subfigure[Recovered Energy]{
\begin{minipage}[b]{0.3\linewidth}
\label{fig:energy-smm}
\includegraphics[width=1\linewidth]{./figs/smm/energy_triangle}
\end{minipage}
}
\subfigure[Induced Policy]{
\begin{minipage}[b]{0.3\linewidth}
\label{fig:policy-smm}
\includegraphics[width=1\linewidth]{./figs/smm/triangle}
\end{minipage}
}


\vspace{-7pt}
\caption{(a) Heuristically-designed samples from target state marginal distribution. (b) The recovered energy by EBIL, representing the density of the demonstrations, where the darker color represent the lower energy and higher rewards. (c) The induced policy using the state-only reward constructed from the energy as shown in (b). The energy value is in a range of $[0,1]$ since we use \textit{sigmoid} for the last layer of the DEEN network on this task.}
\vspace{-2pt}
\label{fig:ablation-energy}
\end{figure*}


\begin{figure*}[htbp]

\centering
\vspace{-40pt}
\includegraphics[width=1\linewidth]{./figs/curves-energy.pdf}
\vspace{-60pt}
\caption{Energy evaluation curves on different mujoco tasks trained by sub-optimal demonstrations , where the red line represents for the average energy estimation on expert data and the blue is for random trajectories, which contain 100 trajectories separately. Note that lower energy values correspond to higher rewards. The energy value is in a range of $[-1,1]$ since we use \textit{tanh} for the last layer of the DEEN network on this task.}
\vspace{-3pt}
\label{fig:curves-energy}
\end{figure*}

==> papers/7-conclusion.tex <==
\section{Conclusion}

In this paper, we propose Energy-Based Imitation Learning (EBIL), which shows that it is feasible to compute a fixed reward function via directly estimating the expert's energy to help agents learn from the demonstrations, which breaks out of the traditional iterative IRL paradigm. We further discuss the relation of our method with Maximum Entropy Inverse Reinforcement Learning (MaxEnt IRL) and reveal that these methods are actually two sides of the same coin. We conduct quantitative and qualitative evaluations in multiple tasks, showing that the meaningful reward can finally lead to comparable performance of EBIL against previous Imitation Learning (IL) algorithms. For future work, we can try different energy estimation methods for expert demonstrations, and exploring more possibilities to utilize EBM to help the agent to learn in different reinforcement learning tasks as state-only learning. It is also intriguing to expand EBIL into multi-agent environments and construct interpretative reward signals for multi-agent learning.


==> papers/discuss-old.tex <==
\section{Discussions}

Our method shows a strong relation with both MaxEnt RL methods and MaxEnt IRL methods. The major difference is that we choose to directly estimate the energy function from expert demonstrations and use it as a surrogate reward function; on the other hand, these two typical series of methods treat that the reward function or the value function exactly as the energy function. We will discuss the theoretical details in this part.

\subsection{Relations with MaxEnt RL}

Soft-Q Learning (SQL)~\cite{haarnoja2017reinforcement} and Soft Actor-Critic (SAC)~\cite{haarnoja2018soft} are two main approaches of MaxEnt RL, particularly, they propose to use a general energy-based form policy as:
\begin{equation}\label{eq:softq}
    \pi(a_t|s_t) \propto \exp{(-E(s_t, a_t))}
\end{equation}
To connect the policy with soft versions of value functions and Q functions, they set the energy model $E(s_t,a_t) = -\frac{1}{\alpha}Q_{\text{soft}}(s_t,a_t)$ where $\alpha$ is the temperature parameter, such that the policy can be represented with the Q function which hold the highest probability at the action with the highest Q value, which essentially provides a soft version of greedy policy. Thus, one can choose to optimize the soft Q function to obtain the optimal policy by minimizing the expected KL-divergence as shown in \eq{eq:softac}.
\begin{equation}\label{eq:softac}
    J(\pi) = \bbE_{s\sim \rho^s_{\caD}}\left[\kld\left( \pi(\cdot|s) \big \| \frac{\exp{(Q(s,\cdot))}}{Z(s)} \right) \right ]
\end{equation}
where $\rho^s_{\caD}$ is the distribution of previously sampled states and actions, or a replay buffer. Therefore, the second term in the KL-divergence in fact can be regarded as the target or the reference for the policy.

Consider to use the KL-divergence as the distance metric in the general objective of IL shown in \eq{eq:il} with taking a logarithm on each policy, then we get:
\begin{equation}
\begin{aligned}
    \pi^* &= \argmin_\pi \mathbb{E}_{\pi} \left [\kld \left( \pi(\cdot|s) \big \| \piE(\cdot|s)  \right) \right ]\\
\end{aligned}
\end{equation}
If we choose to model the expert policy using the energy form of \eq{eq:softq} then we get:
\begin{equation}
\begin{aligned}\label{eq:softil}
    \pi^* &= \argmin_\pi \mathbb{E}_{\pi}\left [\kld \left( \pi(\cdot|s) \big \| \frac{\exp{(-E_\piE(s,a)})}{Z} \right) \right ]\\
\end{aligned}
\end{equation}

\begin{proposition}
    The IL objective shown in \eq{eq:softil} is equivalent to the EBIL objective shown in \eq{eq:eb-il}.
\end{proposition}
\begin{proof}
    Since \eq{eq:eb-il} is equivalent to \eq{eq:kl-il}, which holds the optimal solution such that $\pi^*=\piE$ according to \prop{prop:kl-il}. Also, it is easy to see that \eq{eq:softil} has the same optimal solution such that $\pi^*=\piE$.
\end{proof}
Thus, \eq{eq:softac} reveals the relation between MaxEnt RL and EBIL. To be more specific, EBIL chooses the energy model learned from expert demonstrations as the target policy. The difference is that MaxEnt RL methods use the Q function to play the role of the energy function to connect with the policy, and iterately update the Q function and the policy, while EBIL directly utilizing the energy function to model the occupancy measure. 
%But in the essence they are similar.
Thus, if we choose SQL or SAC as the RL learning algorithm for our EBIL method, one can either directly set the energy model as the target policy or the reward function to iterately update the policy.

\subsection{Relations with MaxEnt IRL}

MaxEnt IRL seeks to infer the reward function underlying expert demonstrations~\cite{ziebart2008maximum}, which assumes that expert trajectories are sampled by an near-optimal policy under some unknown cost. Formally, MaxEnt IRL models the demonstrations using a Boltzmann distribution~\cite{finn2016connection}, where the energy is given by the reward function $r$:
\iffalse
\begin{equation}
    p(s,a) = \frac{1}{Z}\exp{(r(s,a))}
\end{equation}
where $Z$ is the partition function. 
\fi
\begin{equation}\label{maxent-irl}
    p(\tau) = \frac{1}{Z}\exp{(r(\tau))}
\end{equation}
where $\tau=\{ s_0, a_0, \cdots, s_T, a_T \}$ is a trajectory consisted of state-action pairs and $T$ is its length, $r(\tau)=\sum_{t}r(s_t,a_t)$, $Z$ is the partition function. \eq{maxent-irl} models the density of optimal trajectories. With such a model, experts can generate any sub-optimal trajectories with a probability increases exponentially as the reward goes higher. MaxEnt IRL objective aims to maximize the likelyhood of the expert demonstrations with parameterized reward function $r_\theta(\tau)$, but is needed to estimate the partition function $Z$, which is hard especially in high-dimensional spaces. Typical methods such as \cite{ziebart2008maximum} use dynamic programming to do such things but is still eeconstrained in simple scenarios. As an improvement, Guided Cost Learning (GCL)~\cite{finn2016guided} introduces a iterative sample-based method for estimating $Z$ in the MaxEnt IRL formulation, which alternates between optimizing the reward function with the estimate and optimizing $q(\tau)$ to minimizing the importance sampling estimate:
\begin{equation}
    \begin{aligned}
        \caL_\text{reward}(r) &= \bbE_{\tau \sim p} \left [ -\log p(\tau) \right ]
        = \bbE_{\tau \sim p} [r(\tau)] + \log Z \\
        &= \bbE_{\tau \sim p} [r(\tau)] + \log \left ( \bbE_{\tau\sim q}\left [ \frac{\exp{(r(\tau))}}{q(\tau)} \right ] \right )\\
        \caL_\text{sampler}(q) &= \bbE_{\tau \sim q} \left [ -r(\tau) \right ] + \bbE_{\tau \sim q} \left [ \log q(\tau) \right ]
    \end{aligned}
\end{equation}
The optimal sampling distribution is the demonstration distribution for the cost function. Thus, this training procedure lead to both a learned cost function and a learned policy. To reduce the variance of the importance ratio due to the poor sampling distribution, or the sampling policy $q$, GCL uses $\mu=\frac{1}{2}p+\frac{1}{2}q$ by mixing the demonstration samples with the generative samples:
\begin{equation}
    \begin{aligned}
        \caL_\text{reward}(r) &= \bbE_{\tau \sim p} [r(\tau)] + \log \left ( \bbE_{\tau\sim q}\left [ \frac{\exp{(r(\tau))}}{\frac{1}{2}\tilde{p}(\tau) +  \frac{1}{2}q(\tau)} \right ] \right )
    \end{aligned}
\end{equation}
Notice that the cost function of the sampling policy $\caL_\text{sampler}(q)$  is exactly the objective of the forward MaxEnt RL procedure, which is derived from minimizing the KL-divergence between the demonstration distribution $p(\tau)=\frac{1}{Z}\exp{-r(\tau)}$ and the sampling distribution $q(\tau)$. This shows similar point of view of the objective of EBIL shown in \eq{eq:kl-il} and \eq{eq:eb-il}.

However, there are still different between these two methods. First, one should understand that MaxEnt IRL assumes that the expert demonstrations is soft-optimal under some unknown reward function. Thus the reward function has to be optimized via maximizing the likelihood shown in $\caL_\text{reward}(r)$ of expert trajectories in the outer loop. In addition, similarly in MaxEnt RL, MaxEnt IRL connects the probability of the optimal demonstration with the reward function using a Boltzmann distribution by letting the reward function as the energy function. 

On the contrast, EBIL does not make any assumption about the expert data and the reward function, but instead starts from estimating the density of expert trajectories, or the occupancy measure with the energy function. Thus the energy function is optimized with the State-of-The-Art energy estimation methods and is used as a surrogate reward to encourage the agent to imitate the trajectories of the expert.

Therefore, MaxEnt IRL and EBIL can be seen as dual methods in some perspective, but EBIL is much simpler and more efficient than the former since it alleviates the toughness of estimating the partition function and the energy function via maximum likelihood using a sample policy, which has to be alternatively updated in a inner loop, by directly estimating the energy function from demonstrations in advance in a denoising or score matching framework as the surrogate reward to guide the policy learning. 

As a supplementary statement, \cite{finn2016connection} shows how to apply GANs into MaxEnt IRL modeling and further reveals the close relationship between GCL and GAIL where GAIL adopts simpler forms for both the discriminator and the generator. Thus all of these methods including our EBIL show strong connections among each other. 
%We will compare these methods from different dimension in \se{seq:irl}.
